A Framework for Designing Fair Ubiquitous Computing Systems

Over the past few decades, ubiquitous sensors and systems have been an integral part of humans' everyday life. They augment human capabilities and provide personalized experiences across diverse contexts such as healthcare, education, and transportation. However, the widespread adoption of ubiquitous computing has also brought forth concerns regarding fairness and equitable treatment. As these systems can make automated decisions that impact individuals, it is essential to ensure that they do not perpetuate biases or discriminate against specific groups. While fairness in ubiquitous computing has been an acknowledged concern since the 1990s, it remains understudied within the field. To bridge this gap, we propose a framework that incorporates fairness considerations into system design, including prioritizing stakeholder perspectives, inclusive data collection, fairness-aware algorithms, appropriate evaluation criteria, enhancing human engagement while addressing privacy concerns, and interactive improvement and regular monitoring. Our framework aims to guide the development of fair and unbiased ubiquitous computing systems, ensuring equal treatment and positive societal impact.

==> 2-background.tex <==
\section{Background and Related Work}
\label{sec:background}

In this section, we first review existing literature on algorithmic fairness, both within the UbiComp community and related fields (Section \ref{related_work:algorithmic_fairness}). We then discuss the challenges and limitations of existing approaches in assessing fairness in UbiComp (Section \ref{related_work:challenge}). 

\subsection{Algorithmic fairness}\label{related_work:algorithmic_fairness}

Machine learning has been increasingly used in both the public and private sectors for making decisions that have real consequences on people's lives, such as diagnosing diseases ~\cite{saria2010integration, sweatt2019discovery} and recognizing physical or psychological human activities~\cite{kwon2020imutube, peng2018aroma}. While these algorithms are intended to improve people's lives, they are often not immune to biases and may bring additional harm to marginalized communities. For instance, algorithms for medical image analysis trained on datasets of privileged groups may have unacceptable 
 levels of performance on unprivileged ones, further exacerbating health disparities~\cite{larrazabal2020gender}. 

There is an emerging body of research that has started to investigate the fairness of algorithmic systems in ubiquitous computing~\cite{xu2022survey, yfantidou2023beyond}. Prior research has indicated that algorithmic bias can originate from imbalanced datasets or model selection. For instance, Larrazaba \etal found that when an imbalanced dataset across gender groups is used to train X-ray image diagnosis, the resulting algorithm consistently underperforms on unprivileged gender groups~\cite{larrazabal2020gender}. Forde \etal~\cite{forde2021model} further examined how model selection can influence algorithmic bias by training two different models with comparable overall performances but disparate performances between males and females. 

Fairness-aware machine learning research has abstracted fairness notions from the real-world context (e.g., equalized odds~\cite{hardt2016equality}, demographic parity, individual fairness~\cite{dwork2012fairness, joseph2016fairness}) and developed fair algorithms accordingly~\cite{corbett2017algorithmic, kleinberg2016inherent}. For example, demographic parity entails a fair algorithm having a parity of positive classification rates across a fixed number of protected groups, while individual fairness in~\cite{dwork2012fairness} requires treating similar individuals similarly. In light of these fairness metrics, researchers have examined algorithmic fairness across a variety of sensitive attributes individually or combined, including gender, age, race, socioeconomic status, sexual orientation, nationality, etc. However, it remains to be explored how these fairness metrics can translate into the context of ubiquitous computing.

Existing research has also summarized three approaches to mitigate potential biases against sensitive groups in algorithms in medical domains. First, pre-processing mechanisms can be used to modify datasets before training prediction algorithms, so that the distribution of privileged and unprivileged groups is similar. Commonly used techniques include dataset re-sampling~\cite{puyol2021fairness}, dataset mix-up~\cite{seyyed2020chexclusion}, and data augmentation. Second, in-process mechanisms can be used to modify ML algorithms to account for fairness during training time, such as adding a regularization term to the objective function that penalizes biases against sensitive groups~\cite{sarhan2020fairness, pakzad2022circle}. Finally, post-processing mechanisms perform post-processing of the output classification to make prediction fairer. 

\subsection{Challenges and Limitations of Algorithmic Fairness in UbiComp}\label{related_work:challenge}



==> fig_tab_alg/demographics.tex <==
\begin{table}[htb!]
    \centering
    \small
    \caption{\textbf{Demographics of Sensitive Attributes.}}
   \renewcommand{\arraystretch}{1}
   \resizebox{0.65\textwidth}{!}{
\begin{tabular}[t]{l|l|rrrr}
\hline \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell[c]{Sensitive\\ Attributes}}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell[c]{(Un)protected \\ Groups}}}} & \multicolumn{4}{c}{\textbf{Number (\%)}} \\\cline{3-6} %& \multicolumn{4}{c}{\textbf{(Min, Max)}}\\\cline{3-18}
         & & \makecell[c]{\textbf{DS1}} & \makecell[c]{\textbf{DS2}} & \makecell[c]{\textbf{DS3}} & \makecell[c]{\textbf{DS4}} \\\hline
         \multirow{2}{*}{Gender} & Non-male & 95 (68\%) & 102 (50\%) & 71 (55\%) &  121 (65\%) \\   
         & Male & 44 (32\%) & 101 (50\%) & 59 (45\%) & 64 (35\%) \\\hline
         \multirow{3}{*}{Race} & Asian & 67 (48\%) & 97 (48\%) & 72 (55\%) & 99 (54\%)  \\
         % & Non-Asian & 72 (52\%) &  &  &  & 
         %  &  &  &  \\
         & Biracial & 
         19 (14\%) & 22 (11\%) & 9 (7\%) & 18 (10\%)  \\
          % & Non-Biracial & 120 (86\%) &  &  &  & 
          % &  &  &  \\
         & White & 
         44 (32\%) & 68 (34\%) & 39 (30\%) & 48 (26\%) \\\hline
          % & Non-White & &  &  &  & 
          % &  &  &  \\\hline
        \multirow{2}{*}{\makecell[l]{First-gen \\ College Student}} & First-gen & 
        44 (32\%) & 62 (31\%) & 45 (35\%) & 67 (36\%) \\
         & Non-first-gen & 
         95 (68\%) & 141 (69\%) & 85 (65\%) & 118 (64\%) \\\hline
         \multirow{2}{*}{\makecell[l]{Sexual \\Orientation}} & Non-heterosexual & 
         17 (12\%) & 15 (7\%) & 22 (17\%) & 39 (21\%) \\ 
         & Heterosexual & 
         122 (88\%) & 188 (93\%) & 108 (83\%) & 146 (79\%) \\\hline
         \multirow{2}{*}{\makecell[l]{Mother's \\ Education}} & Below Bachelor & 
         56 (40\%) & 81 (40\%) & 57 (44\%) & 72 (39\%) \\
         & Bachelor or Higher & 
         83 (60\%) & 122 (60\%) & 73 (56\%) & 113 (61\%) \\\hline
         \multirow{2}{*}{\makecell[l]{Father's \\ Education}} & Below Bachelor & 
         55 (40\%) & 78 (38\%) & 59 (45\%) & 85 (46\%) \\
         & Bachelor or Higher & 
         84 (60\%) & 125 (62\%) & 71 (55\%) & 100 (54\%) \\\hline
         \multirow{2}{*}{\makecell[l]{Immigration \\ Status}} & Immigrant & 
         31 (22\%) & 52 (26\%) & 33 (25\%) & 43 (23\%) \\
         & Non-immigrant & 
         108 (78\%) & 151 (74\%) & 97 (75\%) & 142 (77\%) \\\hline
       
    \end{tabular}}
    \label{tab:demo}
\end{table}

==> fig_tab_alg/fig_boxplot.tex <==
\begin{figure}[htb!]
    \centering 
    \caption{Comparisons of Depression (BDI-II) scores for different groups of four datasets. The red dotted line indicates the cutoff point (i.e., 13) for BDI-II scores, which is used to distinguish between students with at least mild depressive symptoms (BDI-II score >=13) and those without (BDI-II < 13). Significance levels after Benjamini-Hochberg (B-H) correction are marked with an asterisk (*$p<0.05$) in red on the subplot. First-gen, BA, and HET represent first-generation college students, bachelor, and heterosexual, respectively.}\label{fig_BDI2}
    \subfloat[DS1 (Year 2018, Pre-COVID)]{\includegraphics[scale=0.36]{figures/boxplot_DS1.pdf}
    \label{fig:boxplot1}}
    \subfloat[DS2 (Year 2019, Pre-COVID)]{\includegraphics[scale=0.36]{figures/boxplot_DS2.pdf}
    \label{fig:boxplot2}}
\end{figure}

\begin{figure}[ht]\ContinuedFloat
    \centering
    \subfloat[DS3 (Year 2020, COVID Year)]{\includegraphics[scale=0.36]{figures/boxplot_DS3.pdf}
    \label{fig:boxplot3}}
    \subfloat[DS4 (Year 2021, COVID Year)]{\includegraphics[scale=0.36]{figures/boxplot_DS4.pdf}
    \label{fig:boxplot4}}
\end{figure}

==> fig_tab_alg/fig_demos.tex <==
\begin{figure}[htb!]
    \centering
    \includegraphics[scale=0.22]{figures/demographics.png}
    \caption{Percentage of each group within each sensitive sub-attribute. The protected group for each sensitive sub-attribution is shaded in dark colors, while the unprotected group is shaded in light colors. Non-male includes women, transgender individuals, and genderqueer individuals, and non-heterosexual includes homosexual, bisexual, and asexual individuals.}
    \label{fig:demo}
\end{figure}

==> fig_tab_alg/replication_results.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.36]{figures/replication_results.png}
    \caption{Replication results. DS1 and DS2 were used in prior work \cite{xu2023globem} and DS3 and DS4 are newly reported in this study. Performance comparison of the algorithms on DS1 and DS2 allows for replication analysis, while evaluation on DS3 and DS4 provides additional insights into the algorithmic fairness. $\Delta$ represents the difference between our results and prior reported results. \han{need to reframe}}
    \label{fig:replication_results}
\end{figure}

==> fig_tab_alg/tab_acc_w_t_demo.tex <==
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.1}
   \resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|rr|rr|rr|rr|}\hline
&& \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}}        & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}}        & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}}        & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}}        \\\cline{3-10}
\multirow{-2}{*}{}& \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
% & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.034 & \cellcolor[HTML]{F4CCCC}0.044 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.011 & 0.180& 0.033& \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 \\
% & Father's Education& \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.022 & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.033 & 0.758& 0.089& 0.072& 0.067\\
% & Mother's Education& 0.112& 0.078& 0.269& 0.089& 0.273& 0.044& \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.022 \\
% & Gender           & 0.063& 0.056& \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.022 & 0.161& 0.022& \cellcolor[HTML]{F4CCCC}0.031 & \cellcolor[HTML]{F4CCCC}0.044 \\
% & Immigration Status& 0.087& 0.067& \cellcolor[HTML]{F4CCCC}0.019 & \cellcolor[HTML]{F4CCCC}0.044 & 0.952& 0.100& 0.631& 0.089\\
% & Asian            & \cellcolor[HTML]{F4CCCC}0.015 & \cellcolor[HTML]{F4CCCC}0.033 & 0.189& 0.067& \cellcolor[HTML]{F4CCCC}0.044 & 0.011& 0.945& 0.100\\
% & Biracial         & 0.899& 0.100& 0.085& 0.056& 0.672& 0.078& 0.606& 0.078\\
% & White            & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 & 0.657& 0.100& 0.274& 0.056& 0.069& 0.056\\
% \multirow{-9}{*}{Canzian \etal \cite{canzian2015trajectories}}            & Sexual Orientation& 0.255& 0.089& 0.222& 0.078& 0.622& 0.067& \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.033 \\\hline
% & First-gen College Student & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.022 & 0.079& 0.022& \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.022 \\
% & Father's Education& \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.044 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.033 & 0.678& 0.078& 0.382& 0.089\\
% & Mother's Education& \cellcolor[HTML]{EA9999}0.004 & 0.056& 0.444& 0.100& 0.067& 0.011& \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.033 \\
% & Gender           & 0.305& 0.089& \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.044 & 0.247& 0.044& 0.083& 0.056\\
% & Immigration Status& \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.022 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.011 & 0.507& 0.067& 0.362& 0.078\\
% & Asian            & \cellcolor[HTML]{EA9999}0.005 & 0.067& \cellcolor[HTML]{F4CCCC}0.012 & 0.067& 0.886& 0.089& 0.806& 0.100\\
% & Biracial         & 0.959& 0.100& 0.129& 0.078& 0.130& 0.033& 0.338& 0.067\\
% & White            & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.033 & \cellcolor[HTML]{EA9999}0.009 & 0.056& 0.892& 0.100& 0.075& 0.044\\
% \multirow{-9}{*}{Saeb \etal \cite{saeb2015mobile}}               & Sexual Orientation& 0.138& 0.078& 0.292& 0.089& 0.406& 0.056& \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.011 \\\hline
& First-gen College Student & 0.401& 0.033& 0.152& 0.022& 0.736& 0.056& 0.278& 0.033\\
& Father's Education& 0.820& 0.100& 0.155& 0.033& 0.188& 0.044& 0.649& 0.067\\
& Mother's Education& 0.696& 0.067& 0.260& 0.067& 0.803& 0.078& 0.983& 0.100\\
& Gender           & 0.377& 0.022& \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.011 & 0.776& 0.067& \cellcolor[HTML]{F4CCCC}0.019 & 0.011\\
& Immigration Status& 0.566& 0.044& 0.237& 0.056& 0.868& 0.089& 0.459& 0.056\\
& Asian            & 0.783& 0.089& 0.864& 0.089& 0.074& 0.033& 0.649& 0.067\\
& Biracial         & 0.705& 0.078& 0.597& 0.078& 0.890& 0.100& 0.934& 0.089\\
& White            & 0.681& 0.056& 0.976& 0.100& \cellcolor[HTML]{F4CCCC}0.020 & 0.011& 0.415& 0.044\\
\multirow{-9}{*}{Farhan \etal \cite{farhan2016behavior}}             & Sexual Orientation& 0.158& 0.011& 0.222& 0.044& \cellcolor[HTML]{F4CCCC}0.042 & 0.022& 0.134& 0.022\\\hline
% & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.034 & \cellcolor[HTML]{F4CCCC}0.044 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.022 & 0.507& 0.056& \cellcolor[HTML]{F4CCCC}0.013 & \cellcolor[HTML]{F4CCCC}0.022 \\
% & Father's Education& \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.022 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 & 0.320& 0.022& 0.167& 0.044\\
% & Mother's Education& 0.112& 0.078& \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.044 & 0.052& 0.011& \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.011 \\
% & Gender           & 0.063& 0.056& \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.033 & 0.785& 0.089& 0.718& 0.089\\
% & Immigration Status& 0.087& 0.067& 0.852& 0.078& 0.426& 0.044& 0.628& 0.078\\
% & Asian            & \cellcolor[HTML]{F4CCCC}0.015 & \cellcolor[HTML]{F4CCCC}0.033 & 0.095& 0.056& 1.000& 0.100& 0.783& 0.100\\
% & Biracial         & 0.899& 0.100& 0.942& 0.100& 0.341& 0.033& 0.482& 0.056\\
% & White            & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 & 0.433& 0.067& 0.609& 0.067& 0.114& 0.033\\
% \multirow{-9}{*}{Wahle \etal \cite{wahle2016mobile}}              & Sexual Orientation& 0.255& 0.089& 0.858& 0.089& 0.684& 0.078& 0.537& 0.067\\\hline
& First-gen College Student & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.021 & \cellcolor[HTML]{F4CCCC}0.022 & 0.499& 0.089& 0.964& 0.100\\
& Father's Education& \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.022 & \cellcolor[HTML]{F4CCCC}0.026 & \cellcolor[HTML]{F4CCCC}0.033 & 0.285& 0.056& 0.767& 0.078\\
& Mother's Education& \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.033 & \cellcolor[HTML]{F4CCCC}0.019 & 0.011& 0.117& 0.033& 0.871& 0.089\\
& Gender           & 0.955& 0.100& 0.409& 0.089& 0.484& 0.078& 0.064& 0.022\\
& Immigration Status& 0.719& 0.078& 0.534& 0.100& 0.745& 0.100& \cellcolor[HTML]{F4CCCC}0.049 & 0.011\\
& Asian            & 0.939& 0.089& 0.359& 0.078& 0.415& 0.067& 0.735& 0.067\\
& Biracial         & 0.436& 0.056& 0.272& 0.067& 0.269& 0.044& 0.184& 0.044\\
& White            & 0.072& 0.044& 0.150& 0.056& \cellcolor[HTML]{F4CCCC}0.035 & 0.011& 0.573& 0.056\\
\multirow{-9}{*}{Lu \etal \cite{lu2018joint}}& Sexual Orientation& 0.707& 0.067& 0.097& 0.044& \cellcolor[HTML]{F4CCCC}0.036 & 0.022& 0.106& 0.033\\\hline
% & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.033 & \cellcolor[HTML]{F4CCCC}0.033 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.022 & 0.183& 0.067& \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.022 \\
% & Father's Education& \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.022 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.033 & 0.184& 0.078& 0.067& 0.056\\
% & Mother's Education& 0.441& 0.078& 0.389& 0.100& \cellcolor[HTML]{F4CCCC}0.027 & 0.022& \cellcolor[HTML]{F4CCCC}0.012 & \cellcolor[HTML]{F4CCCC}0.033 \\
% & Gender           & 0.277& 0.056& \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.044 & 0.358& 0.089& 0.093& 0.067\\
% & Immigration Status& \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.026 & 0.011& 0.889& 0.100\\
% & Asian            & 0.750& 0.089& \cellcolor[HTML]{EA9999}0.009 & 0.056& 0.670& 0.100& 0.793& 0.089\\
% & Biracial         & 0.930& 0.100& 0.140& 0.078& 0.136& 0.056& 0.291& 0.078\\
% & White            & 0.202& 0.044& \cellcolor[HTML]{F4CCCC}0.012 & 0.067& 0.063& 0.033& 0.060& 0.044\\
% \multirow{-9}{*}{Wang \etal \cite{wang2018tracking}}               & Sexual Orientation& 0.309& 0.067& 0.307& 0.089& 0.064& 0.044& \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.011 \\\hline
% & First-gen College Student & 0.239& 0.056& 0.180& 0.044& 0.211& 0.033& 0.447& 0.067\\
% & Father's Education& 0.277& 0.067& 0.991& 0.100& 0.298& 0.056& 0.215& 0.011\\
% & Mother's Education& \cellcolor[HTML]{F4CCCC}0.023 & 0.011& 0.116& 0.011& 0.991& 0.100& 0.269& 0.033\\
% & Gender           & 0.172& 0.033& 0.256& 0.056& 0.607& 0.078& 0.216& 0.022\\
% & Immigration Status& 0.219& 0.044& 0.642& 0.089& 0.506& 0.067& 0.978& 0.100\\
% & Asian            & 0.718& 0.100& 0.161& 0.033& \cellcolor[HTML]{F4CCCC}0.021 & \cellcolor[HTML]{F4CCCC}0.022 & 0.342& 0.044\\
% & Biracial         & 0.574& 0.089& 0.148& 0.022& \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.011 & 0.739& 0.089\\
% & White            & 0.151& 0.022& 0.256& 0.067& 0.275& 0.044& 0.542& 0.078\\
% \multirow{-9}{*}{Xu \etal - Interpretable \cite{xu2019leveraging}} & Sexual Orientation& 0.330& 0.078& 0.556& 0.078& 0.838& 0.089& 0.392& 0.056\\\hline
% & First-gen College Student & 0.548& 0.044& 0.058& 0.044& 0.696& 0.056& 0.294& 0.044\\
% & Father's Education& 0.737& 0.078& 0.603& 0.089& 0.910& 0.089& 0.975& 0.100\\
% & Mother's Education& 0.564& 0.056& 0.580& 0.067& 0.319& 0.033& 0.681& 0.078\\
% & Gender           & 0.355& 0.022& 0.313& 0.056& 0.910& 0.089& 0.842& 0.089\\
% & Immigration Status& 0.742& 0.089& \cellcolor[HTML]{F4CCCC}0.023 & \cellcolor[HTML]{F4CCCC}0.033 & 0.185& 0.022& 0.629& 0.067\\
% & Asian            & 0.751& 0.100& \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.022 & \cellcolor[HTML]{F4CCCC}0.012 & 0.011& 0.171& 0.033\\
% & Biracial         & 0.343& 0.011& 0.589& 0.078& 0.855& 0.078& 0.066& 0.022\\
% & White            & 0.428& 0.033& \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.011 & 0.396& 0.044& 0.343& 0.056\\
% \multirow{-9}{*}{Xu \etal - Personalized \cite{xu2022survey}}  & Sexual Orientation& 0.658& 0.067& 0.731& 0.100& 0.825& 0.067& 0.066& 0.011\\
% & First-gen College Student & 0.826& 0.067& 0.238& 0.044& 0.107& 0.033& \cellcolor[HTML]{F4CCCC}0.027 & 0.011\\\hline
% & Father's Education& 0.956& 0.089& 0.750& 0.078& 0.052& 0.022& 0.115& 0.044\\
% & Mother's Education& 0.366& 0.044& 0.106& 0.033& \cellcolor[HTML]{F4CCCC}0.038 & 0.011& 0.074& 0.022\\
% & Gender           & 0.992& 0.100& 0.916& 0.089& 0.472& 0.067& 0.582& 0.078\\
% & Immigration Status& 0.946& 0.078& 0.073& 0.022& 0.812& 0.100& 0.879& 0.100\\
% & Asian            & 0.261& 0.033& 0.378& 0.056& 0.645& 0.078& 0.647& 0.089\\
% & Biracial         & 0.170& 0.022& 0.057& 0.011& 0.239& 0.044& 0.496& 0.067\\
% & White            & 0.654& 0.056& 0.921& 0.100& 0.279& 0.056& 0.090& 0.033\\
% \multirow{-9}{*}{Chikersal \etal \cite{chikersal2021detecting}}          & Sexual Orientation& 0.027& 0.011& 0.416& 0.067& 0.660& 0.089& 0.129& 0.056  \\\hline   
\end{tabular}}
\caption{Accuracy. \han{to fill}}\label{tab:acc_w_t_demo}
\end{table}

==> fig_tab_alg/tab_fnr_w_t_demo.tex <==
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.1}
   \resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|rr|rr|rr|rr|}\hline
&& \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}}        & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}}        & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}}        & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}}        \\\cline{3-10}
\multirow{-2}{*}{}& \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
%      & First-gen College Student                  & 1.000& 0.056& 0.155& 0.044& 0.181& 0.022& 0.470& 0.044\\
%      & Father's Education& 1.000& 0.056& 0.147& 0.033& 0.687& 0.089& 0.494& 0.067\\
%      & Mother's Education& 1.000& 0.056& 0.423& 0.078& 0.576& 0.067& 0.565& 0.078\\
%      & Gender            & 1.000& 0.056& 0.128& 0.022& 0.145& 0.011& 0.312& 0.022\\
%      & Immigration Status& 1.000& 0.056& 0.228& 0.056& 0.443& 0.044& 0.565& 0.078\\
%      & Asian             & 1.000& 0.056& 0.350& 0.067& 0.562& 0.056& 0.080& 0.011\\
%      & Biracial          & 1.000& 0.056& 0.739& 0.100& 0.576& 0.067& 0.777& 0.100\\
%      & White             & 1.000& 0.056& \cellcolor[HTML]{F4CCCC}0.037 & 0.011& 0.805& 0.100& 0.328& 0.033\\
% \multirow{-9}{*}{Wahle \etal \cite{wahle2016mobile}}               & Sexual Orientation& 1.000& 0.056& 0.714& 0.089& 0.255& 0.033& 0.471& 0.056\\\hline
%      & First-gen College Student                  & 0.315& 0.056& 1.000& 0.056& 0.452& 0.067& 0.416& 0.067\\
%      & Father's Education& \cellcolor[HTML]{F4CCCC}0.016 & \cellcolor[HTML]{F4CCCC}0.022 & 1.000& 0.056& 0.266& 0.044& \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.022 \\
%      & Mother's Education& 0.069& 0.033& 1.000& 0.056& 0.870& 0.100& 0.119& 0.056\\
%      & Gender            & 0.113& 0.044& 1.000& 0.056& 0.408& 0.056& 0.635& 0.078\\
%      & Immigration Status& 0.381& 0.078& 1.000& 0.056& 0.622& 0.089& 0.074& 0.044\\
%      & Asian             & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.011 & 1.000& 0.056& 0.550& 0.078& 1.000& 0.100\\
%      & Biracial          & 0.726& 0.089& 1.000& 0.056& \cellcolor[HTML]{EA9999}0.009 & \cellcolor[HTML]{F4CCCC}0.022 & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.011 \\
%      & White             & 0.378& 0.067& 1.000& 0.056& \cellcolor[HTML]{F4CCCC}0.041 & 0.033& 0.060& 0.033\\
% \multirow{-9}{*}{Saeb \etal \cite{saeb2015mobile}}                 & Sexual Orientation& 0.804& 0.100& 1.000& 0.056& \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.011 & 0.939& 0.089\\\hline
     & First-gen College Student                  & 0.369& 0.056& 0.111& 0.022& 0.503& 0.044& 0.601& 0.078\\
     & Father's Education& 0.083& 0.022& 0.470& 0.078& 0.728& 0.078& 0.408& 0.067\\
     & Mother's Education& 0.302& 0.044& 0.386& 0.067& 0.519& 0.056& \cellcolor[HTML]{F4CCCC}0.025 & 0.011\\
     & Gender            & 0.796& 0.089& 0.381& 0.056& 0.605& 0.067& 0.187& 0.033\\
     & Immigration Status& 0.208& 0.033& 0.371& 0.044& \cellcolor[HTML]{F4CCCC}0.038 & 0.011& 0.289& 0.044\\
     & Asian             & 0.752& 0.078& \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.011 & 0.223& 0.022& 0.704& 0.089\\
     & Biracial          & 0.739& 0.067& 0.975& 0.100& 0.777& 0.089& 0.346& 0.056\\
     & White             & 0.861& 0.100& 0.858& 0.089& 0.307& 0.033& 0.141& 0.022\\
\multirow{-9}{*}{Farhan \etal \cite{farhan2016behavior}}           & Sexual Orientation& \cellcolor[HTML]{F4CCCC}0.049 & 0.011& 0.230& 0.033& 0.878& 0.100& 0.715& 0.100\\\hline
%      & First-gen College Student                  & 1.000& 0.056& 0.200& 0.044& 0.731& 0.067& 0.068& 0.033\\
%      & Father's Education& 1.000& 0.056& 0.898& 0.089& 0.108& 0.011& 0.847& 0.100\\
%      & Mother's Education& 1.000& 0.056& \cellcolor[HTML]{F4CCCC}0.016 & 0.011& 0.173& 0.022& 0.070& 0.044\\
%      & Gender            & 1.000& 0.056& \cellcolor[HTML]{F4CCCC}0.036 & 0.022& 0.211& 0.033& 0.070& 0.044\\
%      & Immigration Status& 1.000& 0.056& 0.092& 0.033& 0.682& 0.056& \cellcolor[HTML]{F4CCCC}0.049 & 0.022\\
%      & Asian             & 1.000& 0.056& 0.949& 0.100& 0.769& 0.078& 0.614& 0.089\\
%      & Biracial          & 1.000& 0.056& 0.485& 0.067& 0.855& 0.100& 0.559& 0.078\\
%      & White             & 1.000& 0.056& 0.590& 0.078& 0.819& 0.089& \cellcolor[HTML]{F4CCCC}0.024 & 0.011\\
% \multirow{-9}{*}{Canzian \etal \cite{canzian2015trajectories}}     & Sexual Orientation& 1.000& 0.056& 0.228& 0.056& 0.342& 0.044& 0.401& 0.067\\\hline
%      & First-gen College Student                  & 0.647& 0.067& 1.000& 0.056& 0.692& 0.078& 0.213& 0.022\\
%      & Father's Education& 0.403& 0.056& 1.000& 0.056& 0.892& 0.100& 0.650& 0.078\\
%      & Mother's Education& 0.928& 0.100& 1.000& 0.056& 0.312& 0.044& 0.577& 0.067\\
%      & Gender            & 0.268& 0.033& 1.000& 0.056& 0.429& 0.056& 0.703& 0.089\\
%      & Immigration Status& 0.715& 0.078& 1.000& 0.056& 0.622& 0.067& 0.768& 0.100\\
%      & Asian             & 0.302& 0.044& 1.000& 0.056& 0.216& 0.022& 0.177& 0.011\\
%      & Biracial          & \cellcolor[HTML]{F4CCCC}0.032 & 0.011& 1.000& 0.056& 0.693& 0.089& 0.418& 0.044\\
%      & White             & 0.059& 0.022& 1.000& 0.056& 0.310& 0.033& 0.428& 0.056\\
% \multirow{-9}{*}{Wang \etal \cite{wang2018tracking}}               & Sexual Orientation& 0.860& 0.089& 1.000& 0.056& 0.145& 0.011& 0.311& 0.033\\\hline
     & First-gen College Student                  & 0.843& 0.078& 0.529& 0.067& 0.535& 0.089& 0.253& 0.056\\
     & Father's Education& 0.916& 0.089& 0.704& 0.100& 0.260& 0.056& 0.160& 0.033\\
     & Mother's Education& \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.033 & \cellcolor[HTML]{F4CCCC}0.020 & 0.011& 0.535& 0.089& 0.634& 0.078\\
     & Gender            & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.022 & 0.200& 0.033& 0.068& 0.022& 0.624& 0.067\\
     & Immigration Status& \cellcolor[HTML]{F4CCCC}0.047 & 0.044& 0.392& 0.044& 0.247& 0.044& 0.246& 0.044\\
     & Asian             & 0.946& 0.100& 0.603& 0.078& \cellcolor[HTML]{F4CCCC}0.050 & 0.011& 0.920& 0.100\\
     & Biracial          & 0.095& 0.056& 0.512& 0.056& 0.535& 0.089& 0.150& 0.022\\
     & White             & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 & 0.679& 0.089& 0.186& 0.033& 0.064& 0.011\\
\multirow{-9}{*}{Lu etal \cite{lu2018joint}}             & Sexual Orientation& 0.218& 0.067& \cellcolor[HTML]{F4CCCC}0.046 & 0.022& 0.301& 0.067& 0.724& 0.089\\\hline
%      & First-gen College Student                  & 0.603& 0.078& \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.022 & 0.284& 0.067& 0.953& 0.100\\
%      & Father's Education& 0.805& 0.100& 0.723& 0.089& 0.978& 0.100& 0.930& 0.089\\
%      & Mother's Education& 0.140& 0.044& 0.482& 0.078& \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.022 & 0.051& 0.011\\
%      & Gender            & \cellcolor[HTML]{F4CCCC}0.033 & 0.011& \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.011 & 0.095& 0.033& 0.142& 0.033\\
%      & Immigration Status& 0.578& 0.067& 0.336& 0.067& 0.575& 0.078& 0.099& 0.022\\
%      & Asian             & 0.081& 0.033& 0.779& 0.100& 0.217& 0.056& 0.561& 0.067\\
%      & Biracial          & 0.711& 0.089& 0.166& 0.044& 0.095& 0.033& 0.207& 0.056\\
%      & White             & 0.252& 0.056& 0.294& 0.056& 0.736& 0.089& 0.146& 0.044\\
% \multirow{-9}{*}{Xu \etal - Interpretable \cite{xu2019leveraging}} & Sexual Orientation& 0.080& 0.022& 0.091& 0.033& \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 & 0.812& 0.078\\\hline
%      & First-gen College Student                  & 0.912& 0.089& 0.866& 0.100& \cellcolor[HTML]{F4CCCC}0.027 & 0.011& 0.361& 0.044\\
%      & Father's Education& 0.320& 0.044& 0.122& 0.033& 0.743& 0.100& \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.011 \\
%      & Mother's Education& 0.335& 0.056& 0.400& 0.067& 0.604& 0.089& 0.239& 0.033\\
%      & Gender            & 0.548& 0.067& 0.307& 0.044& 0.207& 0.056& 0.074& 0.022\\
%      & Immigration Status& 0.844& 0.078& 0.719& 0.078& 0.376& 0.078& 0.654& 0.056\\
%      & Asian             & 0.149& 0.033& 0.831& 0.089& 0.195& 0.044& 0.927& 0.078\\
%      & Biracial          & \cellcolor[HTML]{EA9999}0.009 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.027 & 0.011& 0.995& 0.100\\
%      & White             & 0.060& 0.022& 0.316& 0.056& 0.075& 0.033& 0.661& 0.067\\
% \multirow{-9}{*}{Xu \etal - Personalized \cite{xu2022survey}}      & Sexual Orientation& 0.942& 0.100& 0.107& 0.022& 0.228& 0.067& 0.981& 0.089\\\hline
%      & First-gen College Student                  & 0.745& 0.067& 0.426& 0.056& 0.682& 0.078& \cellcolor[HTML]{F4CCCC}0.019 & 0.011\\
%      & Father's Education& \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.011 & 0.169& 0.033& 0.978& 0.089& 0.598& 0.100\\
%      & Mother's Education& 0.727& 0.056& 0.965& 0.100& 0.991& 0.100& 0.081& 0.056\\
%      & Gender            & 0.892& 0.100& 0.875& 0.089& 0.380& 0.067& 0.140& 0.067\\
%      & Immigration Status& 0.831& 0.078& 0.841& 0.078& 0.327& 0.056& \cellcolor[HTML]{F4CCCC}0.029 & 0.022\\
%      & Asian             & 0.872& 0.089& 0.288& 0.044& 0.095& 0.022& 0.509& 0.089\\
%      & Biracial          & 0.391& 0.033& 0.118& 0.022& \cellcolor[HTML]{F4CCCC}0.019 & 0.011& 0.055& 0.033\\
%      & White             & 0.628& 0.044& \cellcolor[HTML]{F4CCCC}0.016 & 0.011& 0.140& 0.033& 0.486& 0.078\\
% \multirow{-9}{*}{Chikersal \etal \cite{chikersal2021detecting}}    & Sexual Orientation& 0.335& 0.022& 0.778& 0.067& 0.283& 0.044& 0.072& 0.044     \\\hline
\end{tabular}}\label{tab_fnr_w_t_demo}
\caption{FNR.}
\end{table}

==> fig_tab_alg/tab_fpr_w_t_demo.tex <==
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.1}
   \resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|rr|rr|rr|rr|}\hline
&& \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}}        & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}}        & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}}        & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}}        \\\cline{3-10}
\multirow{-2}{*}{}& \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
%     & First-gen College Student              & 1.000& 0.056& \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 & 0.146& 0.044& \cellcolor[HTML]{F4CCCC}0.031 & \cellcolor[HTML]{F4CCCC}0.033 \\
%     & Father's Education & 1.000& 0.056& 0.414& 0.078& 0.440& 0.078& \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.011 \\
%     & Mother's Education & 1.000& 0.056& \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.033 & 0.214& 0.056& \cellcolor[HTML]{F4CCCC}0.023 & 0.022\\
%     & Gender        & 1.000& 0.056& 0.166& 0.067& 0.053& 0.033& 0.084& 0.056\\
%     & Immigration Status & 1.000& 0.056& \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.022 & 0.741& 0.100& 0.626& 0.089\\
%     & Asian         & 1.000& 0.056& 0.861& 0.089& 0.347& 0.067& 0.706& 0.100\\
%     & Biracial      & 1.000& 0.056& 0.134& 0.056& \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.022 & 0.367& 0.067\\
%     & White         & 1.000& 0.056& 0.104& 0.044& \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 & 0.062& 0.044\\
% \multirow{-9}{*}{Wahle \etal \cite{wahle2016mobile}}               & Sexual Orientation & 1.000& 0.056& 0.984& 0.100& 0.606& 0.089& 0.489& 0.078\\ \hline
%     & First-gen College Student              & 0.260& 0.078& 1.000& 0.056& \cellcolor[HTML]{F4CCCC}0.014 & \cellcolor[HTML]{F4CCCC}0.033 & 0.348& 0.044\\
%     & Father's Education & 0.054& 0.033& 1.000& 0.056& 0.528& 0.067& 0.664& 0.078\\
%     & Mother's Education & \cellcolor[HTML]{F4CCCC}0.032 & 0.011& 1.000& 0.056& 0.973& 0.100& 0.672& 0.100\\
%     & Gender        & 0.062& 0.044& 1.000& 0.056& 0.372& 0.056& 0.668& 0.089\\
%     & Immigration Status & 0.276& 0.089& 1.000& 0.056& 0.550& 0.078& 0.563& 0.067\\
%     & Asian         & 0.089& 0.067& 1.000& 0.056& 0.206& 0.044& \cellcolor[HTML]{F4CCCC}0.028 & 0.022\\
%     & Biracial      & 0.076& 0.056& 1.000& 0.056& \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.022 & 0.135& 0.033\\
%     & White         & \cellcolor[HTML]{F4CCCC}0.050 & 0.022& 1.000& 0.056& \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.015 & 0.011\\
% \multirow{-9}{*}{Saeb \etal \cite{saeb2015mobile}}                 & Sexual Orientation & 0.792& 0.100& 1.000& 0.056& 0.821& 0.089& 0.460& 0.056\\ \hline
    & First-gen College Student              & 0.219& 0.033& \cellcolor[HTML]{F4CCCC}0.018 & 0.011& 0.892& 0.100& 0.085& 0.033\\
    & Father's Education & 0.939& 0.100& 0.218& 0.022& \cellcolor[HTML]{EA9999}0.010 & \cellcolor[HTML]{F4CCCC}0.022 & \cellcolor[HTML]{F4CCCC}0.038 & 0.022\\
    & Mother's Education & 0.246& 0.044& 0.646& 0.067& 0.370& 0.067& \cellcolor[HTML]{F4CCCC}0.022 & 0.011\\
    & Gender        & 0.334& 0.078& 0.571& 0.056& 0.348& 0.044& 0.346& 0.067\\
    & Immigration Status & 0.620& 0.089& 0.646& 0.078& 0.600& 0.078& 0.423& 0.078\\
    & Asian         & 0.067& 0.022& 0.484& 0.044& 0.362& 0.056& 0.635& 0.089\\
    & Biracial      & 0.272& 0.067& 0.402& 0.033& \cellcolor[HTML]{F4CCCC}0.027 & \cellcolor[HTML]{F4CCCC}0.033 & 0.133& 0.056\\
    & White         & \cellcolor[HTML]{F4CCCC}0.042 & 0.011& 0.707& 0.089& \cellcolor[HTML]{EA9999}0.010 & \cellcolor[HTML]{F4CCCC}0.011 & 0.112& 0.044\\
\multirow{-9}{*}{Farhan \etal \cite{farhan2016behavior}}           & Sexual Orientation & 0.260& 0.056& 0.929& 0.100& 0.784& 0.089& 0.945& 0.100\\ \hline
%     & First-gen College Student              & 1.000& 0.056& 0.066& 0.056& 0.481& 0.033& 0.972& 0.100\\
%     & Father's Education & 1.000& 0.056& 0.260& 0.078& 0.243& 0.022& 0.546& 0.067\\
%     & Mother's Education & 1.000& 0.056& \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.022 & 0.726& 0.078& \cellcolor[HTML]{F4CCCC}0.037 & 0.033\\
%     & Gender        & 1.000& 0.056& \cellcolor[HTML]{F4CCCC}0.024 & \cellcolor[HTML]{F4CCCC}0.033 & 0.582& 0.044& \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.011 \\
%     & Immigration Status & 1.000& 0.056& \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.012 & 0.011& 0.511& 0.056\\
%     & Asian         & 1.000& 0.056& 0.893& 0.100& 0.726& 0.078& \cellcolor[HTML]{F4CCCC}0.045 & 0.044\\
%     & Biracial      & 1.000& 0.056& 0.075& 0.067& 0.646& 0.067& 0.962& 0.089\\
%     & White         & 1.000& 0.056& 0.063& 0.044& 0.622& 0.056& \cellcolor[HTML]{F4CCCC}0.030 & 0.022\\
% \multirow{-9}{*}{Canzian \etal \cite{canzian2015trajectories}}     & Sexual Orientation & 1.000& 0.056& 0.542& 0.089& 0.861& 0.100& 0.547& 0.078\\ \hline
%     & First-gen College Student              & 0.548& 0.044& 0.083& 0.044& 0.704& 0.089& 0.207& 0.044\\
%     & Father's Education & 0.929& 0.089& 0.082& 0.033& \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 & 0.536& 0.078\\
%     & Mother's Education & 0.549& 0.056& 0.277& 0.089& 0.605& 0.078& 0.298& 0.056\\
%     & Gender        & 0.688& 0.067& \cellcolor[HTML]{F4CCCC}0.043 & 0.022& 0.488& 0.056& 0.537& 0.089\\
%     & Immigration Status & 0.383& 0.033& \cellcolor[HTML]{F4CCCC}0.018 & 0.011& 0.757& 0.100& 0.426& 0.067\\
%     & Asian         & 0.708& 0.078& 0.185& 0.078& \cellcolor[HTML]{F4CCCC}0.040 & 0.022& \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.011 \\
%     & Biracial      & \cellcolor[HTML]{F4CCCC}0.019 & 0.011& 0.086& 0.056& 0.109& 0.044& 0.094& 0.022\\
%     & White         & 0.071& 0.022& 0.151& 0.067& 0.082& 0.033& 0.560& 0.100\\
% \multirow{-9}{*}{Wang \etal \cite{wang2018tracking}}               & Sexual Orientation & 0.998& 0.100& 0.988& 0.100& 0.574& 0.067& 0.113& 0.033\\ \hline
    & First-gen College Student              & 0.257& 0.044& 1.000& 0.056& 0.100& 0.022& 0.372& 0.067\\
    & Father's Education & 0.618& 0.078& 1.000& 0.056& \cellcolor[HTML]{F4CCCC}0.029 & 0.011& \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 \\
    & Mother's Education & 0.324& 0.056& 1.000& 0.056& 0.556& 0.100& 0.367& 0.056\\
    & Gender        & 0.915& 0.100& 1.000& 0.056& 0.183& 0.044& 0.784& 0.089\\
    & Immigration Status & 0.798& 0.089& 1.000& 0.056& 0.426& 0.078& 0.154& 0.033\\
    & Asian         & \cellcolor[HTML]{F4CCCC}0.019 & \cellcolor[HTML]{F4CCCC}0.022 & 1.000& 0.056& 0.103& 0.033& 0.920& 0.100\\
    & Biracial      & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.011 & 1.000& 0.056& 0.292& 0.067& 0.156& 0.044\\
    & White         & 0.059& 0.033& 1.000& 0.056& 0.259& 0.056& 0.124& 0.022\\
\multirow{-9}{*}{Lu etal \cite{lu2018joint}}             & Sexual Orientation & 0.541& 0.067& 1.000& 0.056& 0.451& 0.089& 0.569& 0.078\\ \hline
%     & First-gen College Student              & 0.969& 0.089& 0.143& 0.044& 0.790& 0.089& 0.063& 0.011\\
%     & Father's Education & 0.460& 0.056& 0.819& 0.100& 0.835& 0.100& 0.199& 0.022\\
%     & Mother's Education & 0.996& 0.100& 0.068& 0.033& 0.290& 0.056& 0.524& 0.033\\
%     & Gender        & 0.320& 0.044& \cellcolor[HTML]{F4CCCC}0.024 & 0.022& 0.132& 0.033& 0.651& 0.056\\
%     & Immigration Status & 0.743& 0.067& 0.156& 0.056& 0.059& 0.011& 0.764& 0.078\\
%     & Asian         & 0.139& 0.033& 0.195& 0.067& 0.780& 0.078& 0.651& 0.044\\
%     & Biracial      & 0.791& 0.078& 0.236& 0.078& 0.112& 0.022& 0.783& 0.089\\
%     & White         & 0.130& 0.022& 0.657& 0.089& 0.228& 0.044& 0.790& 0.100\\
% \multirow{-9}{*}{Xu \etal - Interpretable \cite{xu2019leveraging}} & Sexual Orientation & \cellcolor[HTML]{F4CCCC}0.017 & 0.011& \cellcolor[HTML]{F4CCCC}0.015 & 0.011& 0.398& 0.067& 0.705& 0.067\\ \hline
%     & First-gen College Student              & 0.853& 0.089& 0.310& 0.067& 0.069& 0.011& 0.182& 0.044\\
%     & Father's Education & 0.211& 0.033& 0.861& 0.089& 0.833& 0.089& 0.723& 0.078\\
%     & Mother's Education & 0.212& 0.044& 0.537& 0.078& 0.609& 0.067& 0.178& 0.033\\
%     & Gender        & 0.456& 0.067& 0.221& 0.056& 0.466& 0.056& 0.982& 0.100\\
%     & Immigration Status & 0.249& 0.056& 0.143& 0.044& 0.317& 0.044& 0.940& 0.089\\
%     & Asian         & 0.941& 0.100& \cellcolor[HTML]{F4CCCC}0.045 & 0.033& 0.609& 0.067& 0.342& 0.056\\
%     & Biracial      & 0.076& 0.011& 0.996& 0.100& 0.157& 0.033& \cellcolor[HTML]{F4CCCC}0.036 & 0.022\\
%     & White         & 0.501& 0.078& \cellcolor[HTML]{EA9999}0.010 & \cellcolor[HTML]{F4CCCC}0.022 & 0.881& 0.100& 0.682& 0.067\\
% \multirow{-9}{*}{Xu \etal - Personalized \cite{xu2022survey}}      & Sexual Orientation & 0.130& 0.022& \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.011 & 0.155& 0.022& \cellcolor[HTML]{EA9999}0.010 & \cellcolor[HTML]{F4CCCC}0.011 \\\hline 
%     & First-gen College Student              & 0.725& 0.089& 0.654& 0.078& 0.420& 0.067& \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.011 \\
%     & Father's Education & 0.593& 0.067& 0.910& 0.100& 0.921& 0.100& 0.217& 0.044\\
%     & Mother's Education & 0.483& 0.056& 0.197& 0.056& 0.311& 0.044& 0.537& 0.078\\
%     & Gender        & 0.416& 0.033& \cellcolor[HTML]{F4CCCC}0.050 & 0.033& 0.557& 0.078& 0.653& 0.089\\
%     & Immigration Status & 0.467& 0.044& 0.846& 0.089& 0.327& 0.056& 0.899& 0.100\\
%     & Asian         & 0.600& 0.078& 0.326& 0.067& \cellcolor[HTML]{F4CCCC}0.022 & 0.011& 0.455& 0.067\\
%     & Biracial      & 0.993& 0.100& \cellcolor[HTML]{F4CCCC}0.024 & 0.011& 0.103& 0.033& \cellcolor[HTML]{F4CCCC}0.023 & \cellcolor[HTML]{F4CCCC}0.033 \\
%     & White         & 0.388& 0.022& 0.139& 0.044& \cellcolor[HTML]{F4CCCC}0.030 & 0.022& \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.022 \\
% \multirow{-9}{*}{Chikersal \etal \cite{chikersal2021detecting}}    & Sexual Orientation & 0.285& 0.011& \cellcolor[HTML]{F4CCCC}0.045 & 0.022& 0.654& 0.089& 0.376& 0.056\\ \hline
\end{tabular}}\label{tab_fpr_w_t_demo}
\caption{FPR.}
\end{table}

==> fig_tab_alg/tab_replication.tex <==
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.1}
   \resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|rrr|rrr|r|r|}
\hline
& \multicolumn{3}{c|}{DS1} & \multicolumn{3}{c|}{DS2} & \multicolumn{1}{c|}{DS3}         & \multicolumn{1}{c|}{DS4} \\ \cline{2-9} 
\multirow{-2}{*}{}        & \multicolumn{1}{l|}{Prior results} & \multicolumn{1}{l|}{Our results} & \multicolumn{1}{l|}{Diff ($\Delta$)} & \multicolumn{1}{l|}{Prior results} & \multicolumn{1}{l|}{Our results} & \multicolumn{1}{l|}{Diff ($\Delta$)} & \multicolumn{1}{l|}{Our results} & \multicolumn{1}{l|}{Our results} \\ \hline
Wahle \etal  \cite{wahle2016mobile}     & \multicolumn{1}{r|}{0.526}         & \multicolumn{1}{r|}{0.538}       & \cellcolor[HTML]{D9D2E9}0.012        & \multicolumn{1}{r|}{0.527}         & \multicolumn{1}{r|}{0.518}       & \cellcolor[HTML]{F4CCCC}-0.009       & 0.514           & 0.514           \\ \hline
Saeb \etal \cite{saeb2015mobile}            & \multicolumn{1}{r|}{0.539}         & \multicolumn{1}{r|}{0.539}       & 0.000               & \multicolumn{1}{r|}{0.508}         & \multicolumn{1}{r|}{0.513}       & \cellcolor[HTML]{D9D2E9}0.005        & 0.588           & 0.500           \\ \hline
Farhan \etal \cite{farhan2016behavior}            & \multicolumn{1}{r|}{0.552}         & \multicolumn{1}{r|}{0.552}       & 0.000               & \multicolumn{1}{r|}{0.609}         & \multicolumn{1}{r|}{0.609}       & 0.000               & 0.563           & 0.609           \\ \hline
Canzian \etal \cite{canzian2015trajectories}           & \multicolumn{1}{r|}{0.559}         & \multicolumn{1}{r|}{0.538}       & \cellcolor[HTML]{F4CCCC}-0.021       & \multicolumn{1}{r|}{0.516}         & \multicolumn{1}{r|}{0.516}       & 0.000               & 0.541           & 0.502           \\ \hline
Wang \etal  \cite{wang2018tracking} & \multicolumn{1}{r|}{0.566}         & \multicolumn{1}{r|}{0.565}       & \cellcolor[HTML]{F4CCCC}-0.001       & \multicolumn{1}{r|}{0.500}         & \multicolumn{1}{r|}{0.500}       & 0.000               & 0.577           & 0.516           \\ \hline
Lu \etal \cite{lu2018joint} & \multicolumn{1}{r|}{0.574}         & \multicolumn{1}{r|}{0.574}       & 0.000               & \multicolumn{1}{r|}{0.558}         & \multicolumn{1}{r|}{0.558}       & 0.000               & 0.611           & 0.553           \\ \hline
Xu \etal - Interpretable \cite{xu2019leveraging} & \multicolumn{1}{r|}{0.722}         & \multicolumn{1}{r|}{0.688}       & \cellcolor[HTML]{F4CCCC}-0.034       & \multicolumn{1}{r|}{0.623}         & \multicolumn{1}{r|}{0.667}       & \cellcolor[HTML]{D9D2E9}0.044        & 0.833           & 0.733           \\ \hline
Xu \etal - Personalized \cite{xu2022survey} & \multicolumn{1}{r|}{0.723}         & \multicolumn{1}{r|}{0.753}       & \cellcolor[HTML]{D9D2E9}0.030        & \multicolumn{1}{r|}{0.699}         & \multicolumn{1}{r|}{0.690}       & \cellcolor[HTML]{F4CCCC}-0.009       & 0.791           & 0.686           \\ \hline
Chikersal \etal  \cite{chikersal2021detecting}       & \multicolumn{1}{r|}{0.728}         & \multicolumn{1}{r|}{0.618}       & \cellcolor[HTML]{F4CCCC}-0.110       & \multicolumn{1}{r|}{0.776}         & \multicolumn{1}{r|}{0.670}       & \cellcolor[HTML]{F4CCCC}-0.106       & 0.581           & 0.641           \\ \hline
\end{tabular}}
\caption{Replication Results. Balanced accuracy of the nine depression prediction algorithms on four datasets: DS1 and DS2, which were used in prior work \cite{xu2023globem}, and DS3 and DS4, which are newly reported in this study. The comparison of algorithm performance on DS1 and DS2 ensures the reliability of our fairness evaluation. The $\Delta$ column represents the difference between our replicated results and the previously reported results. The cells highlighted in red indicate that our replicated results are worse than the previously reported results, while the cells highlighted in purple indicate that our replicated results are better.}\label{tab:replication_results}
\end{table}
